Semi-Empirical Modeling of the Atmospheres of the M Dwarf Exoplanet Hosts GJ 832 and GJ 581

Stellar ultraviolet (UV) radiation drives photochemistry, and extreme-ultraviolet (EUV) radiation drives mass loss in exoplanet atmospheres. However, the UV flux is partly unobservable due to interstellar absorption, particularly in the EUV range (100--912 A). It is therefore necessary to reconstruct the unobservable spectra in order to characterize the radiation environment of exoplanets. In the present work, we use a radiative transfer code SSRPM to build one-dimensional semi-empirical models of two M dwarf exoplanet hosts, GJ 832 and GJ 581, and synthesize their spectra. SSRPM is equipped with an extensive atomic and molecular database and full-NLTE capabilities. We use observations in the visible, ultraviolet, and X-ray ranges to constrain atmospheric structures of the modeled stars. The synthesized integrated EUV fluxes are found to be in good agreement with other reconstruction techniques, but the spectral energy distributions (SEDs) disagree significantly across the EUV range. More than 2/3 of the EUV flux is formed above $10^5$ K. We find that the far ultraviolet (FUV) continuum contributes 42--54 % of the entire FUV flux between 1450--1700 A. The comparison of stellar structures of GJ 832 and GJ 581 suggests that GJ 832 is a more magnetically active star, which is corroborated by other activity indicators.

==> journalabbreviations.tex <==

\newcommand\aj{AJ}%        % Astronomical Journal 
\newcommand\araa{ARA\&A}%  % Annual Review of Astron and Astrophys 
\newcommand\apj{ApJ}%    % Astrophysical Journal ++
\newcommand\apjl{ApJL}     % Astrophysical Journal, Letters 
\newcommand\apjs{ApJS}%    % Astrophysical Journal, Supplement 
\newcommand\ao{ApOpt}%   % Applied Optics ++
\newcommand\apss{Ap\&SS}%  % Astrophysics and Space Science 
\newcommand\aap{A\&A}%     % Astronomy and Astrophysics 
\newcommand\aapr{A\&A~Rv}%  % Astronomy and Astrophysics Reviews 
\newcommand\aaps{A\&AS}%    % Astronomy and Astrophysics, Supplement 
\newcommand\azh{AZh}%       % Astronomicheskii Zhurnal 
\newcommand\baas{BAAS}%     % Bulletin of the AAS 
\newcommand\icarus{Icarus}% % Icarus
\newcommand\jrasc{JRASC}%   % Journal of the RAS of Canada 
\newcommand\memras{MmRAS}%  % Memoirs of the RAS 
\newcommand\mnras{MNRAS}%   % Monthly Notices of the RAS 
\newcommand\pra{PhRvA}% % Physical Review A: General Physics ++
\newcommand\prb{PhRvB}% % Physical Review B: Solid State ++
\newcommand\prc{PhRvC}% % Physical Review C ++
\newcommand\prd{PhRvD}% % Physical Review D ++
\newcommand\pre{PhRvE}% % Physical Review E ++
\newcommand\prl{PhRvL}% % Physical Review Letters 
\newcommand\pasp{PASP}%     % Publications of the ASP 
\newcommand\pasj{PASJ}%     % Publications of the ASJ 
\newcommand\qjras{QJRAS}%   % Quarterly Journal of the RAS 
\newcommand\skytel{S\&T}%   % Sky and Telescope 
\newcommand\solphys{SoPh}% % Solar Physics 
\newcommand\sovast{Soviet~Ast.}% % Soviet Astronomy 
\newcommand\ssr{SSRv}% % Space Science Reviews 
\newcommand\zap{ZA}%       % Zeitschrift fuer Astrophysik 
\newcommand\nat{Nature}%  % Nature 
\newcommand\iaucirc{IAUC}% % IAU Cirulars 
\newcommand\aplett{Astrophys.~Lett.}%  % Astrophysics Letters 
\newcommand\apspr{Astrophys.~Space~Phys.~Res.}% % Astrophysics Space Physics Research 
\newcommand\bain{BAN}% % Bulletin Astronomical Institute of the Netherlands 
\newcommand\fcp{FCPh}%   % Fundamental Cosmic Physics 
\newcommand\gca{GeoCoA}% % Geochimica Cosmochimica Acta 
\newcommand\grl{Geophys.~Res.~Lett.}%  % Geophysics Research Letters 
\newcommand\jcp{JChPh}%     % Journal of Chemical Physics 
\newcommand\jgr{J.~Geophys.~Res.}%     % Journal of Geophysics Research 
\newcommand\jqsrt{JQSRT}%   % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand\memsai{MmSAI}% % Mem. Societa Astronomica Italiana 
\newcommand\nphysa{NuPhA}%     % Nuclear Physics A 
\newcommand\physrep{PhR}%       % Physics Reports 
\newcommand\physscr{PhyS}%        % Physica Scripta 
\newcommand\planss{Planet.~Space~Sci.}%  % Planetary Space Science 
\newcommand\procspie{Proc.~SPIE}%      % Proceedings of the SPIE 

\newcommand\actaa{AcA}%  % Acta Astronomica
\newcommand\caa{ChA\&A}%  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{ChJA\&A}%  % Chinese Journal of Astronomy and Astrophysics
\newcommand\jcap{JCAP}%  % Journal of Cosmology and Astroparticle Physics
\newcommand\na{NewA}%  % New Astronomy
\newcommand\nar{NewAR}%  % New Astronomy Review
\newcommand\pasa{PASA}%  % Publications of the Astron. Soc. of Australia
\newcommand\rmxaa{RMxAA}%  % Revista Mexicana de Astronomia y Astrofisica

%% added feb 9, 2016
\newcommand\maps{M\&PS}% Meteoritics and Planetary Science
\newcommand\aas{AAS Meeting Abstracts}% American Astronomical Society Meeting Abstracts
\newcommand\dps{AAS/DPS Meeting Abstracts}% American Astronomical Society/Division for Planetary Sciences Meeting Abstracts


\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 
\let\applopt=\ao 

